A Recursive Partitioning Approach for Dynamic Discrete Choice Modeling in High Dimensional Settings

Dynamic discrete choice models are widely employed to answer substantive and policy questions in settings where individuals' current choices have future implications. However, estimation of these models is often computationally intensive and/or infeasible in high-dimensional settings. Indeed, even specifying the structure for how the utilities/state transitions enter the agent's decision is challenging in high-dimensional settings when we have no guiding theory. In this paper, we present a semi-parametric formulation of dynamic discrete choice models that incorporates a high-dimensional set of state variables, in addition to the standard variables used in a parametric utility function. The high-dimensional variable can include all the variables that are not the main variables of interest but may potentially affect people's choices and must be included in the estimation procedure, i.e., control variables. We present a data-driven recursive partitioning algorithm that reduces the dimensionality of the high-dimensional state space by taking the variation in choices and state transition into account. Researchers can then use the method of their choice to estimate the problem using the discretized state space from the first stage. Our approach can reduce the estimation bias and make estimation feasible at the same time. We present Monte Carlo simulations to demonstrate the performance of our method compared to standard estimation methods where we ignore the high-dimensional explanatory variable set.

==> Algorithms/Algorithm-1.tex <==
\begin{algorithm}
\begin{algorithmic}[1]
  \STATE{Set $\hat{v}_u^0(x_u,j)=0$}
  \WHILE{Not Converged}
    \STATE{Estimate $\hat{v}_s^k(x_s,j)$ using a dynamic discrete choice model and $\hat{v}_u^{k-1}(x_u,j)$ as offset.}
    \STATE{Estimate $\hat{v}_u^k(x_u,j)$ using a high-dimensional maximum likelihood estimation method and $\hat{v}_s^{k}(x_s,j)$ as offset.}
  \ENDWHILE
  \STATE{Estimate $s(.)$ using recursive partitioning and $\hat{v}_u^*(x_u,j)$ as outcome.}
  \STATE{Estimate $f(.)$ and $\alpha$ using discretized state (by $s(.)$) and a dynamic discrete choice model.}
\end{algorithmic}
\caption{State Space Discretization Algorithm}
\label{pseudo:step1}
\end{algorithm}

==> Algorithms/Algorithm.tex <==
\begin{algorithm}
\begin{algorithmic}[1]
  \STATE{$s(x_u)^0={1}$}
  \WHILE{Not Converged}
    \STATE{Estimate $\hat{v}^k(x_s,s(x_u),j)$ using a dynamic discrete choice model}
    \STATE{Estimate $\hat{e}(x_u, j)$ using recursive partitioning such that $v(x_s,x_u,j)=\hat{v}^k(x_s,.,j)+\hat{e}(x_u, j)$ maximize the likelihood.}
    \STATE{Construct $s^k(.)$ using the partitions in $\hat(e)$}
  \ENDWHILE
\end{algorithmic}
\caption{State Space Discretization Algorithm}
\label{pseudo:step1}
\end{algorithm}

==> Figures/fq.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=80mm]{Figures/FiguresFile/fq.png}
    \caption{\label{figure:fq} The replacement cost with respect to $q_1$ and $q_2$.} 
\end{figure}

==> Figures/split.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=80mm]{Figures/FiguresFile/split.png}
    \caption{\label{figure:split} The example of the recursive partitioning scheme. The dashed lines are the potential splits that the algorithm tests, and the thick dashed line is the split that increases the likelihood the most. Each dot specifies an observation.} 
\end{figure}

==> Figures/time_complexity.tex <==
\begin{figure}[!ht]
    \centering
    \subfloat[Example 1]{{\includegraphics[width=6cm]{Figures/FiguresFile/time_complexity_1.png} }}
    \qquad
    \subfloat[Example 2]{{\includegraphics[width=7.5cm]{Figures/FiguresFile/time_complexity_2.png} }}%
    \caption{\label{figure:time_complexity} Two examples of the resulting patterns in the second step's recursive partitioning scheme.} 
\end{figure}

==> Tables/alphaResult.tex <==
\begin{table}[!htbp]
\centering
\footnotesize
\begin{tabular}{l|cc}
\toprule
{\textbf{State Transition Setting}} &    \textbf{Neglect $\mathbf{\Q}$} &  \textbf{Our Algorithm} \\
\hline\hline
     No Transition &       -0.156 (0.004) &     -0.2 (0.002) \\
 Sparse Transition &       -0.164 (0.002) &     -0.2 (0.003) \\
 Random Transition &       -0.169 (0.002) &     -0.2 (0.003) \\
\bottomrule
\end{tabular}
\caption{\label{table:alpharesults} The comparison of the estimated value for $\alpha$. The means and standard deviations are taken from 100 rounds of simulation. The true value for $\alpha$ is -0.2.}
\end{table}

==> Tables/fResult.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{l|c|cccc}
\toprule
{} &    \textbf{Neglect $\mathbf{\Q}$} &  \multicolumn{4}{c}{\textbf{Our Algorithm}} \\
{\textbf{State Transition Setting}} & $f_1$ & $f_1(0)$ & $f_1(1)$ & $f_1(2)$ & $f_1(3)$ \\
\hline\hline
No Transition &    3.716 (0.102) &  3.011 (0.057) &  4.014 (0.125) &  5.026 (0.141) &  5.965 (0.147) \\
Sparse Transition &    3.788 (0.032) &  3.007 (0.050) &  4.003 (0.051) &  5.005 (0.064) &  6.013 (0.077) \\
Random Transition &    3.760 (0.032) &  3.000 (0.044) &  4.004 (0.056) &  5.002 (0.055) &  6.002 (0.063) \\

\bottomrule
\end{tabular}
\caption{\label{table:fresults} The comparison of the estimated replacement cost. The means and standard deviations are taken from 100 rounds of simulation. Our algorithm correctly estimated the four different partitions within $\Q$, and the replacement cost within each of them.}
\end{table}

==> Tables/logistic_loss_comparison_10000.tex <==
\begin{table}
\begin{tabular}{c|ccc|cccc}
\toprule
\textbf{Case} & \textbf{Effect on}  & \textbf{Effect on} & \textbf{Transition} & \multicolumn{4}{c}{\multirow{1}{*}{Model and high-dimensional data type}}\\
\textbf{No.} & \textbf{Purchase}  & \textbf{Price} &    \textbf{in $\Pii^*(\Q)$}  &  Logistic & Neural net &  Logistic & Neural net\\
& \textbf{Utility}   & \textbf{Transition}   & \textbf{Space} & \mathbf{Q}& \mathbf{Q} & $\Pi^*$(\mathbf{Q}) & $\Pi^*$(\mathbf{Q})\\
\midrule
1 & Dissimilar & Dissimilar & No transition & \makecell{0.2949\\0.0031} & \makecell{0.2994\\0.0048} & \makecell{0.2874\\0.0007} & \makecell{0.2849\\0.0001} \\
2 & Dissimilar & Dissimilar & Random transition & \makecell{0.2948\\0.0104} & \makecell{0.2914\\0.0092} & \makecell{0.2678\\0.0012} & \makecell{0.2654\\0.0006} \\
3 & Dissimilar & Dissimilar & Sparse transition & \makecell{0.2223\\0.0116} & \makecell{0.2157\\0.0097} & \makecell{0.1926\\0.0018} & \makecell{0.1871\\0.0008} \\
4 & Dissimilar & Similar & No transition & \makecell{0.3415\\0.0030} & \makecell{0.3440\\0.0033} & \makecell{0.3332\\0.0006} & \makecell{0.3316\\0.0002} \\
5 & Dissimilar & Similar & Random transition & \makecell{0.3181\\0.0063} & \makecell{0.3183\\0.0062} & \makecell{0.3000\\0.0006} & \makecell{0.2998\\0.0006} \\
6 & Dissimilar & Similar & Sparse transition & \makecell{0.3197\\0.0061} & \makecell{0.3200\\0.0056} & \makecell{0.3022\\0.0009} & \makecell{0.3039\\0.0016} \\
7 & Similar & Dissimilar & No transition & \makecell{0.3438\\0.0021} & \makecell{0.3485\\0.0034} & \makecell{0.3400\\0.0008} & \makecell{0.3384\\0.0006} \\
8 & Similar & Dissimilar & Random transition & \makecell{0.3483\\0.0029} & \makecell{0.3525\\0.0044} & \makecell{0.3428\\0.0010} & \makecell{0.3398\\0.0004} \\
9 & Similar & Dissimilar & Sparse transition & \makecell{0.3077\\0.0049} & \makecell{0.3088\\0.0054} & \makecell{0.2998\\0.0018} & \makecell{0.2947\\0.0007} \\
10 & Similar & Similar & No transition & \makecell{0.3567\\0.0015} & \makecell{0.3604\\0.0024} & \makecell{0.3535\\0.0005} & \makecell{0.3521\\0.0001} \\
11 & Similar & Similar & Random transition & \makecell{0.3530\\0.0013} & \makecell{0.3578\\0.0029} & \makecell{0.3500\\0.0004} & \makecell{0.3493\\0.0003} \\
12 & Similar & Similar & Sparse transition & \makecell{0.3488\\0.0013} & \makecell{0.3526\\0.0025} & \makecell{0.3455\\0.0004} & \makecell{0.3443\\0.0002} \\
\bottomrule
\end{tabular}
\caption{\label{table:ccp_loss1} Predictive performance of logistic regression and neural network models using original (\mathbf{Q}) and discretized ($\Pii^*$(\mathbf{Q})) high-dimensional variable set in simulation 1. Each model is evaluated on a dataset with 10{,}000 observations using both cross-entropy loss (top line) and mean squared error (MSE, bottom line). The true probabilities used for evaluation are those generated by the underlying data-generating process. Cross-entropy loss is computed as $-\frac{1}{n} \sum_{i=1}^{n} \left[ p_i \log \hat{p}_i + (1 - p_i) \log (1 - \hat{p}_i) \right]$, and MSE is $\frac{1}{n} \sum_{i=1}^{n} (p_i - \hat{p}_i)^2$.}
\end{table}


==> Tables/sim1_alt_result.tex <==
\begin{sidewaystable}[!htbp]
\centering
\footnotesize
\begin{tabular}{c|ccc|cccc}
\toprule
\textbf{Case} & \textbf{Effect on}  & \textbf{Effect on} & \textbf{Transition} & \multicolumn{4}{c}{\multirow{2}{*}{\textbf{Number of Allowed Partitions}}}\\
\textbf{No.} & \textbf{Replacement}  & \textbf{Mileage} &    \textbf{in $\Pii^*(\Q)$}  &  & \\
& \textbf{Cost}   & \textbf{Transition}   & \textbf{Sapce} & \textbf{1}& \textbf{2} & \textbf{4} & \textbf{6}\\
\midrule
Case 1  &         Dissimilar &     Dissimilar &     No transition &           -0.135 &           -0.173 &           -0.194 &           -0.193 \\
        &                    &             &                   & (-0.144, -0.127) &  (-0.18, -0.167) & (-0.204, -0.187) & (-0.204, -0.186) \\
Case 2  &         Dissimilar &     Dissimilar & Random transition &           -0.149 &           -0.186 &             -0.2 &           -0.199 \\
        &                    &             &                   & (-0.154, -0.142) &  (-0.191, -0.18) & (-0.206, -0.193) & (-0.206, -0.192) \\
Case 3  &         Dissimilar &     Dissimilar & Sparse transition &           -0.123 &           -0.182 &           -0.199 &           -0.199 \\
        &                    &             &                   & (-0.129, -0.118) & (-0.198, -0.167) & (-0.207, -0.191) & (-0.207, -0.191) \\
Case 4  &         Dissimilar &     Similar &     No transition &           -0.165 &           -0.191 &           -0.199 &           -0.198 \\
        &                    &             &                   & (-0.172, -0.158) &   (-0.2, -0.183) &  (-0.207, -0.19) &  (-0.207, -0.19) \\
Case 5  &         Dissimilar &     Similar & Random transition &           -0.171 &           -0.193 &             -0.2 &           -0.199 \\
        &                    &             &                   & (-0.177, -0.162) & (-0.201, -0.184) & (-0.209, -0.192) & (-0.209, -0.192) \\
Case 6  &         Dissimilar &     Similar & Sparse transition &            -0.17 &           -0.096 &           -0.201 &           -0.201 \\
        &                    &             &                   & (-0.176, -0.164) & (-0.119, -0.067) & (-0.211, -0.189) & (-0.211, -0.188) \\
Case 7  &         Similar    &     Dissimilar &     No transition &           -0.178 &           -0.193 &           -0.199 &           -0.199 \\
        &                    &             &                   &  (-0.188, -0.17) & (-0.201, -0.187) & (-0.208, -0.192) & (-0.208, -0.192) \\
Case 8  &         Similar    &     Dissimilar & Random transition &           -0.185 &           -0.197 &             -0.2 &             -0.2 \\
        &                    &             &                   & (-0.194, -0.179) & (-0.205, -0.189) & (-0.208, -0.192) & (-0.207, -0.191) \\
Case 9  &         Similar    &     Dissimilar & Sparse transition &           -0.174 &           -0.236 &             -0.2 &             -0.2 \\
        &                    &             &                   & (-0.182, -0.168) & (-0.247, -0.224) & (-0.209, -0.193) & (-0.209, -0.193) \\
Case 10 &         Similar    &     Similar &     No transition &             -0.2 &           -0.199 &           -0.199 &           -0.198 \\
        &                    &             &                   & (-0.205, -0.192) & (-0.205, -0.192) & (-0.204, -0.189) & (-0.204, -0.188) \\
Case 11 &         Similar    &     Similar & Random transition &             -0.2 &           -0.199 &           -0.199 &           -0.198 \\
        &                    &             &                   & (-0.207, -0.193) & (-0.207, -0.193) & (-0.207, -0.192) & (-0.206, -0.191) \\
Case 12 &         Similar    &     Similar & Sparse transition &           -0.199 &           -0.199 &           -0.198 &           -0.198 \\
        &                    &             &                   & (-0.209, -0.192) & (-0.208, -0.192) &  (-0.208, -0.19) &  (-0.207, -0.19) \\
\bottomrule
\end{tabular}

\caption{\label{table:sim1_alt_result} The estimated mileage maintenance cost, $c_m$, and the 96\% bootstrap confidence interval around the mean in each of the 12 Monte Carlo simulations. Each cell is a result of 100 rounds of simulation for 4 buses. Note that the case where the number of partitions is set to 1 is equivalent to completely neglecting $\Q$. }
\end{sidewaystable}

==> Tables/simple_simulation_res.tex <==
\begin{sidewaystable}[!htbp]
\centering
\footnotesize
\begin{tabular}{c|ccc|cccc|c}
\toprule
\textbf{Case} & \textbf{Effect on}  & \textbf{Effect on} & \textbf{Transition} & \multicolumn{4}{c}{\multirow{2}{*}{Incorporating discretized $\Q$}} & \multicolumn{1}{c}{\multirow{2}{*}{Neglecting $\Q$}}\\
\textbf{No.} & \textbf{Replacement}  & \textbf{Mileage} &    \textbf{in $\Pii^*(\Q)$}  &  & \\
 & \textbf{Cost}   & \textbf{Transition}   & \textbf{Sapce}         &                  $f_{dc}(\pi_1)$ &             $f_{dc}(\pi_2)$ &             $f_{dc}(\pi_3)$ &             $f_{dc}(\pi_4)$ &           {$c_r$}  \\
\midrule
Case 1  &         Dissimilar &     Dissimilar &     No transition &           -6.812 &           -5.845 &           -4.843 &           -4.435 &           -5.408 \\
        &                    &             &                   & (-7.115, -6.589) & (-6.121, -5.635) & (-5.084, -4.642) & (-4.724, -3.908) &  (-5.76, -5.148) \\
Case 2  &         Dissimilar &     Dissimilar & Random transition &           -7.006 &           -6.008 &           -4.998 &           -3.995 &           -4.962 \\
        &                    &             &                   & (-7.179, -6.834) & (-6.132, -5.853) & (-5.165, -4.831) &  (-4.13, -3.852) & (-5.099, -4.846) \\
Case 3  &         Dissimilar &     Dissimilar & Sparse transition &           -7.015 &           -5.987 &           -4.984 &           -3.984 &           -4.886 \\
        &                    &             &                   & (-7.352, -6.773) & (-6.201, -5.804) & (-5.139, -4.846) & (-4.222, -3.773) & (-5.046, -4.766) \\
Case 4  &         Dissimilar &     Similar &     No transition &           -6.975 &           -5.964 &           -4.977 &             -4.0 &           -4.701 \\
        &                    &             &                   &  (-7.252, -6.69) &  (-6.162, -5.74) &  (-5.142, -4.82) &   (-4.13, -3.86) & (-4.906, -4.548) \\
Case 5  &         Dissimilar &     Similar & Random transition &           -7.025 &           -5.996 &           -4.997 &           -3.995 &           -4.661 \\
        &                    &             &                   & (-7.327, -6.775) &  (-6.211, -5.83) & (-5.183, -4.829) & (-4.165, -3.842) & (-4.769, -4.507) \\
Case 6  &         Dissimilar &     Similar & Sparse transition &           -7.061 &           -6.028 &           -5.021 &           -4.012 &           -4.731 \\
        &                    &             &                   & (-7.394, -6.769) & (-6.253, -5.757) & (-5.244, -4.813) & (-4.221, -3.803) & (-4.858, -4.618) \\
Case 7  &         Similar    &     Dissimilar &     No transition &           -5.064 &           -5.019 &           -4.977 &           -4.925 &           -5.323 \\
        &                    &             &                   & (-5.218, -4.901) & (-5.163, -4.857) & (-5.138, -4.811) & (-5.083, -4.732) & (-5.524, -5.115) \\
Case 8  &         Similar    &     Dissimilar & Random transition &           -5.041 &            -5.01 &           -4.986 &           -4.957 &           -5.039 \\
        &                    &             &                   & (-5.191, -4.905) & (-5.151, -4.883) &  (-5.14, -4.856) &  (-5.115, -4.84) &   (-5.221, -4.9) \\
Case 9  &         Similar    &     Dissimilar & Sparse transition &           -5.059 &           -5.021 &           -4.994 &           -4.956 &           -5.045 \\
        &                    &             &                   & (-5.237, -4.905) & (-5.196, -4.854) & (-5.149, -4.847) & (-5.112, -4.812) & (-5.219, -4.864) \\
Case 10 &         Similar    &     Similar &     No transition &           -5.043 &           -4.998 &           -4.963 &           -4.911 &           -4.994 \\
        &                    &             &                   & (-5.196, -4.886) & (-5.131, -4.861) & (-5.086, -4.823) & (-5.039, -4.779) &  (-5.11, -4.869) \\
Case 11 &         Similar    &     Similar & Random transition &           -5.033 &           -4.994 &           -4.975 &           -4.936 &             -5.0 \\
        &                    &             &                   &  (-5.25, -4.874) & (-5.162, -4.851) &  (-5.12, -4.831) & (-5.099, -4.772) & (-5.143, -4.863) \\
Case 12 &         Similar    &     Similar & Sparse transition &           -5.005 &           -4.982 &           -4.964 &           -4.939 &           -4.989 \\
        &                    &             &                   & (-5.166, -4.842) & (-5.118, -4.817) & (-5.102, -4.813) & (-5.094, -4.808) & (-5.129, -4.827) \\
\bottomrule
\end{tabular}
\caption{\label{table:simple_simulation_res} The estimated replacement cost and their 96\% bootstrap confidence interval around the mean in each of the 12 Monte Carlo simulations. Each row is a result of 100 rounds of simulation. }
\end{sidewaystable}

==> Tables/simulation_2_res_match.tex <==
\begin{table}[!htbp]
\centering
\footnotesize
\begin{tabular}{ccc|ccccccc}
\toprule
Number & Transition & $\Pii^*(Q)$  & \multicolumn{7}{c}{\multirow{2}{*}{Value of $\lambda_{rel}$}}\\
of & in $\Pii^*(Q)$ & affect mileage \\
Periods  &  space & transition &    0 &    0.2 & 0.5 &  1 &  2 &    5 &  100 \\
\midrule
        \multirow{4}{*}{100}  &              Sparse &               Yes &  1.39 & 4.81 & 8.07 &  9.54 & 10.30 & 10.05 &  9.88 \\
         &              Sparse &                No &  1.63 & 6.68 & 9.29 & 10.01 & 10.18 &  9.09 &  7.37 \\
         &              Random &               Yes &  1.86 & 3.43 & 6.10 &  6.32 &  6.03 &  5.21 &  3.83 \\
         &              Random &                No &  2.54 & 2.63 & 2.71 &  3.01 &  3.19 &  2.87 &  0.00 \\
        \midrule
        \multirow{4}{*}{400}  &              Sparse &               Yes &  3.62 & 6.74 & 8.73 &  9.68 & 10.25 & 10.14 & 10.16 \\
         &              Sparse &                No &  5.04 & 8.42 & 9.40 &  9.98 & 10.08 &  9.44 &  7.56 \\
         &              Random &               Yes &  4.16 & 6.20 & 7.36 &  7.06 &  6.55 &  5.56 &  4.24 \\
         &              Random &                No &  7.28 & 7.45 & 7.47 &  7.55 &  7.64 &  7.28 &  0.29 \\
\bottomrule
\end{tabular}
\caption{\label{table:simulation_2_res_match} The number of matched partition between the true discretization and the discretization generated by different values of $\lambda_{rel}$ in different data-generating processes. Discretization on the training data.}
\end{table}

==> Tables/simulation_2_res_score.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{c|ccc|ccccccc}
\toprule
Case & Number & Transition & $\Pii^*(Q)$  & \multicolumn{7}{c}{\multirow{2}{*}{Value of $\lambda_{rel}$}}\\
No. & of & in $\Pii^*(Q)$ & affects mileage \\
& Periods  &  space & transition &    0 &    0.2 & 0.5 &  1 &  2 &    5 &  100 \\
\midrule
Case 1 &         \multirow{4}{*}{100} &              Sparse &               Yes &  -3722 &  -3481 &  -3274 &  -3121 &  -2977 &  -2864 &  \textbf{-2766} \\
Case 2 &          &              Sparse &                No &  -3762 &  -3536 &  -3407 &  -3323 &  -3245 &  \textbf{-3200} &  -3228 \\
Case 3 &          &              Random &               Yes &  -3743 &  -3762 &  \textbf{-3730} &  -3768 &  -3831 &  -3913 &  -4062 \\
Case 4 &          &              Random &                No &  \textbf{-3698 }&  -3781 &  -3867 &  -3959 &  -4063 &  -4192 &  -4373 \\
         \midrule
Case 5 &         \multirow{4}{*}{400} &              Sparse &               Yes & -13287 & -12969 & -12606 & -12239 & -11864 & -11519 & \textbf{-11217} \\
Case 6 &          &              Sparse &                No & -13815 & -13650 & -13469 & -13264 & -13059 & \textbf{-12909} & -12987 \\
Case 7 &          &              Random &               Yes & \textbf{-13518} & -13620 & -13693 & -13770 & -13863 & -13974 & -14187 \\
Case 8 &          &              Random &                No & \textbf{-13613} & -13921 & -14231 & -14542 & -14856 & -15177 & -15556 \\
\bottomrule
\end{tabular}
\caption{\label{table:simulation_2_res_score} The calculated score for different values of $\lambda_{rel}$ in different data-generating processes. A bigger $\lambda_{rel}$ is better when there is more information in the state transition data. Scores are averaged over the 100 different partitioning schemes and shown for the validation data.}
\end{table}
